Generative View Synthesis: From Single-view Semantics to Novel-view Images

Content creation, central to applications such as virtual reality, can be a tedious and time-consuming. Recent image synthesis methods simplify this task by offering tools to generate new views from as little as a single input image, or by converting a semantic map into a photorealistic image. We propose to push the envelope further, and introduce Generative View Synthesis (GVS), which can synthesize multiple photorealistic views of a scene given a single semantic map. We show that the sequential application of existing techniques, e.g., semantics-to-image translation followed by monocular view synthesis, fail at capturing the scene's structure. In contrast, we solve the semantics-to-image translation in concert with the estimation of the 3D layout of the scene, thus producing geometrically consistent novel views that preserve semantic structures. We first lift the input 2D semantic map onto a 3D layered representation of the scene in feature space, thereby preserving the semantic labels of 3D geometric structures. We then project the layered features onto the target views to generate the final novel-view images. We verify the strengths of our method and compare it with several advanced baselines on three different datasets. Our approach also allows for style manipulation and image editing operations, such as the addition or removal of objects, with simple manipulations of the input style images and semantic maps respectively. Visit the project page at https://gvsnet.github.io.

==> 2_preliminaries.tex <==
%!TEX root = main.tex
\label{sec:preliminaries}
\section{Preliminaries}
\subsection{Multi-Plane Image Representation}

In this section we will provide a brief summary of the MPI scene representation and rendering. MPIs represent a scene as a set of planes $D$ planes, $P  = \{\left[n_{1}^{T}, d_{1} \right], $ $ \left[n_{2}^{T}, d_{2} \right], \dots \left[n_{D}^{T}, d_{D} \right]\}$, where $n_{i}$ and $d_{i}$ stand for the plane normal and distance of the $i-th$ plane, in a reference camera coordinate system. The number of planes is a hyper-parameter that controls the trade-off between scene representation capability and computational complexity of the MPI. Each MPI plane has color and opacity values associated to it. We denote multi-plane color as $C = \{C_{0}, C_{1}, \dots, C_{D}\}$ where $C_{i} \in R^{W \times H \times C}$, and opacity as $\alpha = \{\alpha_{0}, \alpha_{1}, \dots, \alpha_{D}\}$ where $\alpha_{i} \in [0,1]^{W \times H}$ for $i \in [1, 2, \dots, D]$. 
\subsection{MPI Rendering}
Let's use $K^{r}$ and $K^{t}$ to denote the intrinsics of the reference and target cameras, repspectively. The relative pose of the target camera w.r.t the the reference camera is expressed as $\theta=[R|T]$, where $R$ is a rotation matrix and $T$ is a translation vector; $\theta$ is $SE(3)$ transformation from the reference to the target camera. As the MPI representation is composed of planes, therefore, it permits planar homography warping of the $C$ and $\alpha$ from the source camera to the target camera. Each plane $i$ induces its own unique homography matrix, $H_{i}$ and a warping function $W_{i}$ associated with $H_{i}$. The calculation of the homography matrix for the $i-th$ plane is given in Equation~\ref{eqn:homography}, for a formal dicsussion of planar homographies refer ~\cite{zisserman_book}. $K^{-r}$ in Equation~\ref{eqn:homography} refers to the inverse of the source camera intrinsics. 
\begin{equation}
    H_{i} = K^{t} \; \begin{bmatrix} R^{T} + \frac{R^{T}\, t\, n_{i}^{T} \, R^{T}}{-d - n_{i} \, R^{T} \, t} \end{bmatrix} \; K^{-r}
    \label{eqn:homography}
\end{equation}

Rendering the scene from the target camera is done in two steps: first $C$ and $\alpha$ are warped to the target camera as follows, $C^{t}_{i} = W_{i}(C_{i})$, $\alpha_{i}^{t} = W_{i}(\alpha_{i})$. Then, the novel view~(in color) $\hat{X}^{t}_{c}$ is computed by alpha compositing $C^{t}$ using $\alpha^{t}$, in a back to front manner. The back-to-front alpha composition could be expressed mathematically as shown in Equation~\ref{eqn:back_to_front}.
\begin{equation}
\hat{X}_{c}^{t} = \sum_{z=1 \dots D} {\begin{bmatrix}
W_{z}(C_{z}) W_{z}(\alpha_{z}) \prod_{j=1}^{z-1}{\begin{bmatrix}
1-W_{j}(\alpha_{j})

\end{bmatrix}}
\end{bmatrix}}
\label{eqn:back_to_front}
\end{equation} 


==> images/figure_4/results_table.tex <==
%!TEX root = ../../main.tex

% Math to compute the sizes
\newlength{\one}
\setlength{\one}{1pt}
\newcommand{\fitscale}{.9}

\newlength{\numcrops}
\setlength{\numcrops}{6pt}

\newlength{\tgt}
\setlength\tgt{\textwidth*\ratio{\one}{\numcrops}}

\captionsetup[subfigure]{labelformat=empty}
\centering

% First row
% Semantic map
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_5_Ours_input_seg_real.png}}\
% Ground truth with box
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_5_Ours_style.png}}~~
% Method 1
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_5_CVS_target_rgb_fake.png}}\
% Method 2
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_5_SM_target_rgb_fake.png}}\
% Method 3
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_5_AF_target_rgb_fake.png}}\
% Method 4
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_5_Ours_target_rgb_fake.png}}\
\\ \vspace{-3mm}


% Second row
% Semantic map
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_0_Ours_input_view_seg_real.png}}\
% Ground truth with box
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_0_Ours_input_view_rgb_real.png}}~~
% Method 1
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_0_CVS_view_10_target_rgb_fake.png}}\
% Method 2
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_0_SM_view_10_target_rgb_fake.png}}\
% Method 3
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_0_AF_view_10_target_rgb_fake.png}}\
% Method 4
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_0_Ours_view_10_target_rgb_fake.png}}\
\\ \vspace{-3mm}


% Third row
% Semantic map
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_2_Ours_input_view_seg_real.png}}\
% Ground truth with box
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_2_Ours_input_view_rgb_real.png}}~~
% Method 1
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_2_CVS_view_05_target_rgb_fake.png}}\
% Method 2
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_2_SM_view_05_target_rgb_fake.png}}\
% Method 3
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_2_AF_view_05_target_rgb_fake.png}}\
% Method 4
\subfloat{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_2_Ours_view_05_target_rgb_fake.png}}\
\\ \vspace{-3mm}


% Last row
% Semantic map
\subfloat[Semantic]{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_3_Ours_input_seg_real.png}}\
% Ground truth with box
\subfloat[RGB]{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_3_AF_style.png}}~~
% Method 1
\subfloat[CVS~\cite{contvs}]{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_3_CVS_target_rgb_fake.png}}\
% Method 2
\subfloat[SM~\cite{zhou2018stereo}]{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_3_SM_target_rgb_fake.png}}\
% Method 3
\subfloat[AF~\cite{appflow}]{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_3_AF_target_rgb_fake.png}}\
% Method 4
\subfloat[Ours]{\includegraphics[width=\fitscale\tgt]{images/figure_4/imgs/row_3_Ours_target_rgb_fake.png}}
